Computing Left Eigenvalues of Quaternion Matrices

We present a practical Newton-based method for computing left eigenvalues of quaternion matrices. It uses only standard real/complex linear-algebra kernels via embeddings and applies to matrices of any size. Extensive tests on literature examples and benchmark ensembles, together with a compact MATLAB reference implementation, demonstrate reproducible, certificate-based computations up to size 64x64, including the detection of multiple spherical components and non-generic phenomena such as more than n isolated left eigenvalues and left-spectrum deficiency.

==> arxiv_submitted_stamp_LAA.tex <==
% arxiv_submitted_stamp_LAA.tex
% ------------------------------------------------------------
% First-page overlay stamp for arXiv submissions (CC BY 4.0).
% Put this file next to your main .tex and \input it.
% Then call \ArxivSubmittedStampOverlay right after \begin{document}.
% ------------------------------------------------------------

\RequirePackage{eso-pic}
\RequirePackage{xcolor}
\RequirePackage{tikz}

% ---- EDIT THESE FOUR LINES ----
\providecommand{\ArxivStampSubmittedTo}{Linear Algebra and its Applications}
\providecommand{\ArxivStampSubmittedDate}{February 1, 2026}
\providecommand{\ArxivStampVersion}{arXiv preprint (submitted manuscript)}
\providecommand{\ArxivStampFunding}{This work was co-funded by the European Union under the project RO\-BO\-PROX (reg. no. CZ.02.01.01/00/22\_008/0004590).}
% --------------------------------

% Optional extra one-liner (leave empty if not needed)
\providecommand{\ArxivStampExtra}{}

\newcommand{\ArxivSubmittedStampOverlay}{%
  \AddToShipoutPictureFG*{%
    \begin{tikzpicture}[remember picture,overlay]
      \node[
        anchor=south,
        inner sep=0pt
      ] at ([yshift=14mm]current page.south) {%
        \begin{minipage}{0.97\paperwidth}
          \setlength{\fboxsep}{6pt}%
          \colorbox{black!6}{%
            \parbox{0.97\paperwidth}{%
              \scriptsize
              \textbf{CC BY 4.0.}\;
              \ArxivStampVersion.\;
              Submitted to \textit{\ArxivStampSubmittedTo} on \ArxivStampSubmittedDate.\;\\
              \textbf{Funding:} \ArxivStampFunding%
              \ifx\ArxivStampExtra\empty\else\; \ArxivStampExtra\fi
            }%
          }%
        \end{minipage}%
      };
    \end{tikzpicture}%
  }%
}

